A Survey on Label-efficient Deep Image Segmentation: Bridging the Gap between Weak Supervision and Dense Prediction

The rapid development of deep learning has made a great progress in image segmentation, one of the fundamental tasks of computer vision. However, the current segmentation algorithms mostly rely on the availability of pixel-level annotations, which are often expensive, tedious, and laborious. To alleviate this burden, the past years have witnessed an increasing attention in building label-efficient, deep-learning-based image segmentation algorithms. This paper offers a comprehensive review on label-efficient image segmentation methods. To this end, we first develop a taxonomy to organize these methods according to the supervision provided by different types of weak labels (including no supervision, inexact supervision, incomplete supervision and inaccurate supervision) and supplemented by the types of segmentation problems (including semantic segmentation, instance segmentation and panoptic segmentation). Next, we summarize the existing label-efficient image segmentation methods from a unified perspective that discusses an important question: how to bridge the gap between weak supervision and dense prediction -- the current methods are mostly based on heuristic priors, such as cross-pixel similarity, cross-label constraint, cross-view consistency, and cross-image relation. Finally, we share our opinions about the future research directions for label-efficient deep image segmentation.

==> text_v6/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pics/WeiShen.png}}]{Wei Shen} is a tenure-track Associate Professor at the Artificial Intelligence Institute, Shanghai Jiao Tong University, since October 2020. Before that, he was an Assistant Research Professor at the Department of Computer Science, Johns Hopkins University. His research interests lie in the fields of computer vision, machine learning, deep learning, and medical image analysis. He is an Area Chair for CVPR 2022/2023 and ACCV 2022.
\end{IEEEbiography}
\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{figures/pics/ZelinPeng2.png}}]{Zelin Peng} received the B.S. and M.S. degrees in control science and engineering from the School of Artificial Intelligence, Xidian University, Xi’an, China, in 2019 and 2022, respectively. He is now a Ph.D. student at the Artificial Intelligence Institute, Shanghai Jiao Tong University, Shanghai, China. His current research interest is weakly supervised semantic segmentation.
\end{IEEEbiography}
\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pics/XuehuiWang2.jpg}}]{Xuehui Wang} received the B.S. and M.S. degrees from Shandong University and Sun Yat-sen University, China, in 2018 and 2021, respectively. He is now a Ph.D. candidate at the Artificial Intelligence Institute, Shanghai Jiao Tong University, China. His current research interests include instance segmentation, object detection and weakly supervised segmentation.
\end{IEEEbiography}
\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pics/Huayuwang2.jpeg}}]{Huayu Wang} received the B.S. degree in computer science and technology from the School of Electronic Information and Electrical Engineering, Shanghai Jiao Tong University, Shanghai, China in 2020. He is now a Master student at the Artificial Intelligence Institute, Shanghai Jiao Tong University, Shanghai, China. His current research interest is domain adaptive semantic segmentation.
\end{IEEEbiography}
\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pics/Jiazhong2.jpeg}}]{Jiazhong Cen} received the B.S. degree in computer science and technology from the School of Electronic Information and Electrical Engineering, Shanghai Jiao Tong University, Shanghai, China in 2021. He is now a Master student at the Artificial Intelligence Institute, Shanghai Jiao Tong University, Shanghai, China. His current research interest is unsupervised semantic segmentation.
\end{IEEEbiography}
\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pics/DongshengJiang2.png}}]{Dongsheng Jiang} received his Ph.D. in Biomedical Engineering from Fudan University. He is currently a senior researcher at Huawei Inc. His research interests lie in computer vision and medical image analysis.
\end{IEEEbiography}
\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pics/Lingxi.pdf}}]
{Lingxi Xie} is currently a senior researcher at Huawei Inc. He obtained B.E. and Ph.D. in engineering, both from Tsinghua University, in 2010 and 2015, respectively. He also served as a post-doctoral researcher at the CCVL lab from 2015 to 2019, having moved from the University of California, Los Angeles to the Johns Hopkins University. His research interests lie in computer vision, in particular, the application of deep learning models. His research covers image classification, object detection, semantic segmentation, and other vision tasks. He is also facilitating the application of automated machine learning to the above research fields. Lingxi has published over 90 papers in top-tier international conferences and journals.
\end{IEEEbiography}
\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pics/Xiaokang.png}}]{Xiaokang Yang} (M’00-SM’04-F’19) received the B.S. degree from Xiamen University, Xiamen, China, in 1994, the M.S. degree from the Chinese Academy of Sciences, Shanghai, China, in 1997, and the Ph.D. degree from Shanghai Jiao Tong University, Shanghai, in 2000. From September 2000 to March 2002, he worked as a Research Fellow with the Centre for Signal Processing, Nanyang Technological University, Singapore. From April 2002 to October 2004, he was a Research Scientist with the Institute for Infocomm Research (I2R), Singapore. From August 2007 to July 2008, he visited the Institute for Computer Science, University of Freiburg, Germany, as an Alexander von Humboldt Research Fellow. He is currently a Distinguished Professor with the School of Electronic Information and Electrical Engineering, Shanghai Jiao Tong University. His current research interests include image processing and communication, computer vision, and machine learning. He is an Associate Editor of the IEEE TRANSACTIONS ON MULTIMEDIA and a Senior Associate Editor of the IEEE SIGNAL PROCESSING LETTERS.
\end{IEEEbiography}
\vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pics/Qi.pdf}}] {Qi Tian} (M'96-SM'03-F'16) received his Ph.D. in ECE from University of Illinois at Urbana-Champaign (UIUC) in 2002. He is currently the Chief Scientist in Artificial Intelligence at Huawei Cloud \& AI. He was the Chief Scientist in Computer Vision at Huawei Noah’s Ark Laboratory from 2018-2020. Before he joined Huawei, Dr. Tian was a Full Professor in the Department of Computer Science, the University of Texas at San Antonio (UTSA) (2002-2019). He was listed in the Top 10 of the 2016 Most Influential Scholars in Multimedia by Aminer.org. He is an IEEE Fellow (Class 2016) and Academician of International Eurasian Academy of Sciences (IEAS), 2021.  He received 2017 UTSA President Distinguished Award for Research Achievement, 2016 UTSA Innovation Award in the first category, 2014 Research Achievement Awards from College of Science, UTSA, and 2010 Google Faculty Research Award. Dr. Tian has served as founding member of ICMR, (2009-2014), ACM MM (2009-2012), and International Steering Committee Member for ACM MIR (2006-2010), ACM ICIMCS 2013, ICME 2006 and 2009, PCM 2012, and IEEE International Symposium on Multimedia 2011, chair for ACM Multimedia 2015. He is the Associate Editor of IEEE TMM, TCSVT, ACM TOMM, MMSJ, and MVA.
\end{IEEEbiography}
\vspace{-10mm}


==> text_v6/wxh_backup.tex <==
\begin{figure}
    \centering
    \begin{overpic}[width=\columnwidth]{figures/labels_v4.pdf}
    \put(1.2,98.8){\tiny{Label Type}}
    \put(21,98.8){\tiny{Training Images}}
    
    \put(8.2,84.5){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{10,235,50}{elephant}, \textcolor[RGB]{255,192,0}{mountain}, \textcolor[RGB]{0,251,255}{sky}''}}}
    \put(25.8,84.5){\tiny{\emph{``\textcolor[RGB]{50,20,235}{bird}, \textcolor[RGB]{0,32,96}{bottle}, \textcolor[RGB]{255,60,200}{chair}, \textcolor[RGB]{57,200,245}{table}, \textcolor[RGB]{255,0,130}{grass}, \textcolor[RGB]{0,255,181}{metal}''}}}
    \put(44.1,84.5){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{255,255,0}{tennis racket}''}}}
    
    \put(13,70.8){\tiny{\emph{``unknown''}}}
    \put(31.5,70.8){\tiny{\emph{``unknown''}}}
    \put(46.5,70.8){\tiny{\emph{``unknown''}}}
    
    \put(8.2,56.8){\tiny{\emph{``person, elephant, mountain, sky''}}}
    \put(25.8,56.8){\tiny{\emph{``bird, bottle, chair, table, grass, metal''}}}
    \put(44.1,56.8){\tiny{\emph{``person, tennis racket''}}}
    
    \put(8.2,42.6){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{10,235,50}{elephant}, \textcolor[RGB]{255,192,0}{mountain}, \textcolor[RGB]{0,251,255}{sky}''}}}
    \put(25.8,42.6){\tiny{\emph{``\textcolor[RGB]{50,20,235}{bird}, \textcolor[RGB]{0,32,96}{bottle}, \textcolor[RGB]{255,60,200}{chair}, \textcolor[RGB]{57,200,245}{table}, \textcolor[RGB]{255,0,130}{grass}, \textcolor[RGB]{0,255,181}{metal}''}}}
    \put(44.1,42.6){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{255,255,0}{tennis racket}''}}}
    
    \put(8.2,28.7){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{10,235,50}{elephant}, \textcolor[RGB]{255,192,0}{mountain}, \textcolor[RGB]{0,251,255}{sky}''}}}
    \put(25.8,28.7){\tiny{\emph{``\textcolor[RGB]{50,20,235}{bird}, \textcolor[RGB]{0,32,96}{bottle}, \textcolor[RGB]{255,60,200}{chair}, \textcolor[RGB]{57,200,245}{table}, \textcolor[RGB]{255,0,130}{grass}, \textcolor[RGB]{0,255,181}{metal}''}}}
    \put(44.1,28.7){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{255,255,0}{tennis racket}''}}}
    
    \put(8.2,14.7){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{10,235,50}{elephant}, \textcolor[RGB]{255,192,0}{mountain}, \textcolor[RGB]{0,251,255}{sky}''}}}
    \put(31.5, 14.7){\tiny{\emph{``unknown''}}}
    \put(46.5,14.7){\tiny{\emph{``unknown''}}}
    
    \put(8.2,0.7){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{10,235,50}{elephant}, \textcolor[RGB]{255,192,0}{mountain}, \textcolor[RGB]{0,251,255}{sky}''}}}
    \put(25.8, 0.7){\tiny{\emph{``\textcolor[RGB]{50,20,235}{bird}, \textcolor[RGB]{0,32,96}{bottle}, \textcolor[RGB]{255,60,200}{chair}, \textcolor[RGB]{57,200,245}{table}, \textcolor[RGB]{255,0,130}{grass}, \textcolor[RGB]{0,255,181}{metal}''}}}
    \put(44.1,0.7){\tiny{\emph{``\textcolor[RGB]{235,10,10}{person}, \textcolor[RGB]{255,255,0}{tennis racket}''}}}

    \put(3.3,93.4){\tiny{\textbf{(a)\label{fig:weak_label_dense}}}}
    \put(1.2,92.0){\tiny{\textbf{Full Dense}}}
    \put(2.5,90.6){\tiny{\textbf{Label}}}

    \put(3.3,79.4){\tiny{\textbf{(b)\label{fig:weak_label_no}}}}
    \put(3.2,78.0){\tiny{\textbf{No}}}
    \put(2.5,76.6){\tiny{\textbf{Label}}}
    
    \put(1.5,51.4){\tiny{\textbf{(c)\label{fig:weak_label_coarse}}}}
    \put(0.4,50.0){\tiny{\textbf{Coarse}}}
    \put(0.6,48.6){\tiny{\textbf{Label}}}
    \put(4.5,64){\tiny{Image}}
    \put(4.7,63){\tiny{Level}}
    \put(5,50){\tiny{Box}}
    \put(4.7,49){\tiny{Level}}
    \put(4.1,36){\tiny{Scribble}}
    \put(4.7,35){\tiny{Level}}
    
    \put(3.3,23.4){\tiny{\textbf{(d)\label{fig:weak_label_incomplete}}}}
    \put(1.2,22.0){\tiny{\textbf{Incomplete}}}
    \put(2.5,20.6){\tiny{\textbf{Label}}}
    
    \put(3.3,9.4){\tiny{\textbf{(e)\label{fig:weak_label_noisy}}}}
    \put(2.4,8.0){\tiny{\textbf{Noisy}}}
    \put(2.5,6.6){\tiny{\textbf{Label}}}
    \end{overpic}
    \caption{Examples for each type of weak labels compared with the full dense label.}
    \label{fig:weak_label}
\end{figure}

==> text_v6/xuehui_IS_fewshot.tex <==
%\subsubsection{Few-shot instance segmentation}

%Few-shot instance segmentation is a special case of semi-supervised segmentation. According to the definition in~\cite{WSIS_MetaRCNN_ICCV_2019}, the training data for this problem are divided into two sets. One is the set of  base categories $C_{base}$, where a large number of training images with full dense labels are provided, the other is the set of novel categories $C_{novel}$ where only a few training images are provided with full dense labels.   

%we can assume that there are base categories $C_{base}$ where a large amount of dense supervisions for objects are provided and novel categories $C_{novel}$ where only a handful of labeled objects and several unlabeled objects are given for each class. The target of this task is to segment unlabeled objects from novel categories through learning on limited labeled data with the same classes and a large amount of data with the different classes. The main possible ways and their difficulties in this task are two aspects: 1) If we first train a segmentation model only using data from $C_{base}$ and then Fine-tuning it on $C_{novel}$, limited labeled data in $C_{novel}$ would lead to an overfitting problem and thus reduce the generalization ability. 2) If we adopt labeled data from $C_{base}$ and $C_{novel}$ simultaneously, an extreme unbalance issue would occur. Recently, to remedy these two obstacles, some works~\cite{WSIS_MetaRCNN_ICCV_2019, WSIS_iMTFA_2021_CVPR, WSIS_FGN_CVPR_2020, WSIS_FAPIS_2021_CVPR} are proposed in this setting by exploiting cross-images priors.

%\noindent \emph{5.1.2.1 Few-shot instance segmentation from cross-image relation}
%In this setting, cross-image relation indicates that same objects within different images should share similar low-level shape distributions or high-level semantic embeddings. Based on this relation, limited labeled data in novel categories are utilized to extract class-attentive vectors to re-parameterize the segmentation model.

%Meta R-CNN~\cite{WSIS_MetaRCNN_ICCV_2019} and FGN~\cite{WSIS_FGN_CVPR_2020} are two similar Mask RCNN based methods that employ the concept of meta-learning to handle this task. In these two methods, meta categories $\mathcal{C}_{meta}$ are randomly sampled from $\mathcal{C}_{base} \bigcup \mathcal{C}_{novel}$ at each iteration and each class in meta contains $K$ images. Meta R-CNN designed a predictor-head remodeling network which shares the same backbone with Mask RCNN to infer class-attentive vectors for meta categories. These vectors can be seen as guided information and are adopted on RoI feature maps to remodel features through performing a channel-wise soft-attention operation. The following steps for detection head and segmentation head are same as Mask RCNN. FGN claimed that Meta R-CNN embedded the 
%class-attentive vectors into the RoI features, which undesirably enforces components for different tasks, \emph{i.e.}, detection, classification, segmentation, to share the same guidance. Thus, in FGN, guided information are separately injected into the RPN, detection head and segmentation head with different formatting. A special training strategy that first only taking $\mathcal{C}_{base}$ as training data to pretrain the network and then utilizing $\mathcal{C}_{meta}$ as training data to finetune the network is adopted in Meta R-CNN and FGN.

==> text_v6/xuehui_IS_scribble_level.tex <==
\subsubsection{Instance segmentation from scribble-level labels}
